Connecting Kaporin's condition number and the Bregman log determinant divergence

This paper presents some theoretical results relating the Bregman log determinant matrix divergence to Kaporin's condition number. These can be viewed as nearness measures between a preconditioner and a given matrix, and we show under which conditions these two functions coincide. We also give examples of constraint sets over which it is equivalent to minimise these two objectives. We focus on preconditioners that are the sum of a positive definite and low-rank matrix, which were developed in a previous work. These were constructed as minimisers of the aforementioned divergence, and we show that they are only a constant scaling from also minimising Kaporin's condition number. We highlight connections to information geometry and comment on future directions.

==> background.tex <==
\section{Background}


\subsection{Information Geometry}

Recall the following from \cite{amari2016information}.

We begin with a definition:
\begin{definition}
The Bregman matrix divergence \cite{bregman1967relaxation} $\Divergence_\phi:\domain \phi\times\relint \domain\phi\rightarrow [0, \infty)$
associated with a proper, continuously-differentiable, strictly convex seed function $\phi$ is defined as follows:
\begin{align*}
    \Divergence_\phi(X,Y) & = \phi(X) - \phi(Y) - \langle \nabla\phi(Y), X - Y\rangle.
\end{align*}
The log determinant matrix divergence, induced by $\phi(x) = -\log\det X$, is given by
\begin{equation}\label{eq:BregmanLogDetDivergence}
\BregmanLogDet(X, Y) = \trace{XY\inv} - \logdet{XY\inv} - n,
\end{equation}
where in this case $\domain \phi = \Snpp$.
\end{definition}

\begin{definition}
The Bregman matrix divergence $\Divergence_\phi:\domain \phi\times\relint \domain\phi\rightarrow [0, \infty)$
associated with a proper, continuously-differentiable, strictly convex 
\emph{seed} function $\phi$ is defined as follows:
\begin{align*}
    \Divergence_\phi(X,Y) & = \phi(X) - \phi(Y) - \Tr{\nabla\phi(Y)\Hermitian (X-Y)}.
\end{align*}
\end{definition}
It is invariant to congruence transformations, i.e. for $X,Y\in\Snpp$ and invertible $P$ we have
\[
\BregmanLogDet(X,Y) = \BregmanLogDet(P\Hermitian X P, P\Hermitian Y P).
\]

Bregman divergences induced by convex seed functions $\phi$ give rise to a dually
flat (affine) structure. Let $\phi^\star$ denote the Fenchel-Legendre conjugate of
$\phi$:
\begin{equation}\label{eq:phi:star}
\phi^\star (x) = \max_{\eta}\; \{ \langle \eta, x\rangle - \phi(\eta)\},
\end{equation}
for some appropriate inner product $\langle \cdot, \cdot\rangle$.
The \emph{dual divergence} $\Divergence_{\phi^\star}$ 
associated with the divergence $\Divergence$ is given by
\begin{equation}\label{eq:dual_divergence}
\Divergence_{\phi^\star}(x, y) = \phi^\star(x) - \phi^\star(y) - \langle\nabla\phi^\star(y), x-y\rangle.
\end{equation}

\begin{theorem}[Geodesic and dual geodesic projections]\label{prop:geodesic_projections}
When $C$ is a flat submanifold of a dually flat manifold $M$, the
\textbf{dual geodesic projection} $P_C^\star$ of $P$ onto $C$ is unique
and given by:
\[
P_C^\star = \arg\min_{R\in C} \Divergence (P, R).
\]
Dually, when $C$ is a \emph{dual} flat submanifold of a dually flat
manifold $M$, the \textbf{geodesic projection} $P_C$ of $P$ onto
$C$ is unique and given by:
\[
P_C = \arg\min_{R\in C} \Divergence^\star (P, R),
\]
where $\Divergence^\star$ is the dual divergence of $\Divergence$.
\end{theorem}
\begin{proof}
See \cite[Theorem 1.5]{amari2016information}.
\end{proof}

\begin{theorem}
When the dual geodesic between $A$ and $B$ is orthogonal to the geodesic
between $B$ and $C$, then
\[
\Divergence(A, C) = \Divergence(A, B) + \Divergence(B, C).
\]
\end{theorem}
We seek to apply this in our preconditioning framework. For our principal
manifold of interest we have:

\begin{theorem}[{\cite[Section 3.7]{nielsen2020elementary}}]
$M = \Snpp$ is a dually flat manifold.
\end{theorem}
%\begin{proof}
%\todo{TODO.}
%\end{proof}
Note also that $M\inv = \{ Y\inv \given Y \in M\}$, which is isomorphic
to $M$, is also dually flat.

\subsection{The log determinant matrix divergence}

Let $\phi(X) = - \ln \det (X)$ be the seed function associated with
\[
D_\phi(A, B) = \trace{AB\inv} - \ln \det(AB\inv) - n.
\]
The dual affine coordinates are
\[
X^\star = \nabla\phi(X) = - X\invtransp.
\]
The dual seed function is defined via Legendre transformation:
\[
\phi^\star(X^\star) = \max_\eta \trace{\eta X^\star} - \phi(\eta),
\]
which simplifies to
\[
\phi^\star(X^\star) = \trace{\nabla\phi\inv(X^\star) X^\star} - \phi(\nabla\phi\inv(X^\star)).
\]
We have
\[
\nabla\phi\inv(X^\star) = X = - (X^\star)\invtransp,
\]
so
\[
\phi^\star(X^\star) = -n - \ln\det(-X^\star),
\]
so the domain of the dual affine variables is $-\Snpp$. This induces
a dual divergence on $-\Snpp \times -\Snpp$:
\[
D_\phi^\star(\Theta, \Sigma) = \phi^\star(\Theta) - \phi^\star(\Sigma) - \langle \nabla\phi^\star(\Sigma), \Theta - \Sigma\rangle.
\]
We note that
\[
D_\phi(A, B) = D_\phi^\star(B^\star, A^\star).
\]
We verify by looking at the right-hand side:
\begin{align*}
D_\phi^\star(B^\star, A^\star)
& = \phi^\star(B^\star) - \phi^\star(A^\star) - \langle \nabla\phi^\star(A^\star), B^\star - A^\star\rangle\\
& = - n - \ln\det (-B^\star) + n + \ln\det (-A^\star) - \trace{- (A^\star)\invtransp (B^\star - A^\star)}\\
& = \ln\det (A^\star (B^\star)\inv) - \trace{- (A^\star)\invtransp (B^\star - A^\star)}\\
& = \ln\det (A^\star (B^\star)\inv) - n + \trace{(A^\star)\invtransp B^\star}\\
& = \ln\det (A\inv B) - n + \trace{A B\inv}\\
& = - \ln\det (A B\inv) - n + \trace{A B\inv}\\
& = D_\phi(A, B).
\end{align*}

Note that this also means
\[
D_\phi(A, B) = D_\phi(B^\star, A^\star).
\]


==> info_geom.tex <==
\section{Interpreting preconditioning using information geometry}

We have so far established a connection between the Bregman log determinant divergence
and the convergence of PCG. Motivated by the numerical results in \cite{bock2023new} 
we now explore the intimate connection between the Bregman divergence and information
geometry.

Recall the following from \cite{amari2016information}. We begin with a definition:
\begin{definition}
The Bregman matrix divergence \cite{bregman1967relaxation} $\Divergence_\phi:\domain \phi\times\relint \domain\phi\rightarrow [0, \infty)$
associated with a proper, continuously-differentiable, strictly convex seed function $\phi$ is defined as follows:
\begin{align*}
    \Divergence_\phi(X,Y) & = \phi(X) - \phi(Y) - \langle \nabla\phi(Y), X - Y\rangle.
\end{align*}
The log determinant matrix divergence, induced by $\phi(x) = -\log\det X$, is given by
\begin{equation}\label{eq:BregmanLogDetDivergence}
\BregmanLogDet(X, Y) = \trace{XY\inv} - \logdet{XY\inv} - n,
\end{equation}
where in this case $\domain \phi = \Snpp$.
\end{definition}

\begin{definition}
The Bregman matrix divergence $\Divergence_\phi:\domain \phi\times\relint \domain\phi\rightarrow [0, \infty)$
associated with a proper, continuously-differentiable, strictly convex 
\emph{seed} function $\phi$ is defined as follows:
\begin{align*}
    \Divergence_\phi(X,Y) & = \phi(X) - \phi(Y) - \Tr{\nabla\phi(Y)\Hermitian (X-Y)}.
\end{align*}
\end{definition}
It is invariant to congruence transformations, i.e. for $X,Y\in\Snpp$ and invertible $P$ we have
\[
\BregmanLogDet(X,Y) = \BregmanLogDet(P\Hermitian X P, P\Hermitian Y P).
\]

Bregman divergences induced by convex seed functions $\phi$ give rise to a dually
flat (affine) structure. Let $\phi^\star$ denote the Fenchel-Legendre conjugate of
$\phi$:
\begin{equation}\label{eq:phi:star}
\phi^\star (x) = \max_{\eta}\; \{ \langle \eta, x\rangle - \phi(\eta)\},
\end{equation}
for some appropriate inner product $\langle \cdot, \cdot\rangle$.
The \emph{dual divergence} $\Divergence_{\phi^\star}$ 
associated with the divergence $\Divergence$ is given by
\begin{equation}\label{eq:dual_divergence}
\Divergence_{\phi^\star}(x, y) = \phi^\star(x) - \phi^\star(y) - \langle\nabla\phi^\star(y), x-y\rangle.
\end{equation}

\begin{theorem}[Geodesic and dual geodesic projections]\label{prop:geodesic_projections}
When $C$ is a flat submanifold of a dually flat manifold $M$, the
dual geodesic projection $P_C^\star$ of $P$ onto $C$ is unique
and given by:
\[
P_C^\star = \arg\min_{R\in C} \Divergence (P, R).
\]
Dually, when $C$ is a \emph{dual} flat submanifold of a dually flat
manifold $M$, the \textbf{geodesic projection} $P_C$ of $P$ onto
$C$ is unique and given by:
\[
P_C = \arg\min_{R\in C} \Divergence^\star (P, R),
\]
where $\Divergence^\star$ is the dual divergence of $\Divergence$.
\end{theorem}
\begin{proof}
See \cite[Theorem 1.5]{amari2016information}.
\end{proof}

\begin{theorem}
When the dual geodesic between $A$ and $B$ is orthogonal to the geodesic
between $B$ and $C$, then
\[
\Divergence(A, C) = \Divergence(A, B) + \Divergence(B, C).
\]
\end{theorem}
We seek to apply this in our preconditioning framework. For our principal
manifold of interest we have:

\begin{theorem}[{\cite[Section 3.7]{nielsen2020elementary}}]
$M = \Snpp$ is a dually flat manifold.
\end{theorem}
%\begin{proof}
%\todo{TODO.}
%\end{proof}
Note also that $M\inv = \{ Y\inv \given Y \in M\}$, which is isomorphic
to $M$, is also dually flat.


\begin{theorem}
We conclude that $P\inv$ is the \emph{dual geodesic projection of $A\inv$ onto the manifold $C_r$}.
\end{theorem}



==> notes.tex <==
\iffalse
We let $M = \mathsf{U}\Pi\mathsf{U}\transp$ denote an eigendecomposition,
and recall $\tilde E = VDV\Hermitian + W\Theta W\Hermitian$, where $VDV\Hermitian$
represents the subspace captured by the Bregman truncation. The eigenvalues
$\Pi$ are given by
\begin{align*}
\pi_i
& = \lambda_i((\alpha WW\Hermitian + V(I_r + D)V\Hermitian)\inv(I + \tilde E))\\
& = \begin{cases}
1 \qquad \text{if} & i \in \BregmanIndexSet{\tilde E} \quad \text{(i.e. in Bregman truncation)},\\
\frac{1 + \theta_i}\alpha & \text{otherwise}.
\end{cases}
%, \quad i=1,\ldots,n.
\end{align*}
We have the eigenvalue $1$ with a multiplicity of (at least) $r$.\\
\fi


==> numerical_results.tex <==
\section{Numerical study}\label{sec:numerical_results}

We conduct several experiments to investigate the effect of the scalars
$c$ and $\alpha$ in the preconditioners \cref{x,y}.




The numerical results shown below were generated using Matlab 
2023b\footnote{The code to reproduce them is available at \url{https://www.github.com/andreasbock/bldp-kaporin-matlab}.}
run on a node featuring two Intel Xeon Processor 2650v4 (12 core, 2.20GHz) with
256 GB memory (16 x 16 GB DDR4-2666).

\subsection{Scaling}
WITHOUT Bregman trunc
with c
with alpha

\subsection{Scaling}
WITH Bregman trunc
with c
with alpha

\iffalse

We select matrices from the SuiteSparse Matrix Collection\footnote{Available
at \url{https://sparse.tamu.edu/}.} \cite{kolodziej2019suitesparse}, as shown in 
\cref{table:ichol_problems}. We consider matrices of modest size in order to compute
BLD truncations and TSVDs with high accuracy.
Some of these correspond to least-squares problems involving $A\in\Rmn$, for which we
consider the corresponding normal equations $S = A\Hermitian b$, for $S=A\Hermitian A$
and a random non-zero $b\in\Realn$. If the matrix is symmetric positive definite,
we simply consider $Sx=b$.\\

\begin{table}
\caption{Test set from the SuiteSparse Matrix Collection. We consider both
symmetric positive definite (SPD) matrices of size $n\times n$ and $m \times n$ matrices
for $m>n$ (transposing if necessary). For the latter, we solve the associated normal 
equations. The number of non-zero entries in the matrix is denoted by $\texttt{nnz}$.
}\label{table:ichol_problems}
\begin{center}
\begin{tabular}{l r r r}
\toprule 
Problem (SPD) & & $n$ & $\texttt{nnz}$\\\midrule
\texttt{HB/bcsstk22} &  & 138 & 696\\
\texttt{HB/lund\_a}  & & 147 & 2449\\
\texttt{HB/bcsstk05}  & & 153 & 2423\\
\texttt{Pothen/mesh2e1}  & & 306 & 2018\\
\texttt{HB/494\_bus}  & & 494 & 1666\\
\texttt{HB/662\_bus}  & & 662 & 2474\\
\texttt{HB/bcsstk08}  & & 1074 & 12960\\
\texttt{HB/1138\_bus} &  & 1138 & 4054\\\midrule
Problem (normal equations) & $m$ & $n$ & $\texttt{nnz}$\\\midrule
\texttt{Meszaros/l9} & 1483 & 244 & 4659\\
\texttt{LPnetlib/lp\_sctap1} & 660 & 300 & 1872\\
\texttt{LPnetlib/lp\_bandm} & 472 & 305 & 2494\\
\texttt{HB/illc1850} & 1850 & 712 & 8636\\
\texttt{LPnetlib/lp\_sctap3} & 3340 & 1480 & 9734\\\bottomrule
\end{tabular}
\end{center}
\end{table}



Theorem 5 tells us...
in practice, we expect this to be different...
\subsection{Setup}
Matrices
Bigfloats in Julia
Links to repository
\subsection{Variable precision $\alpha$}
Why does alpha affect things? where is the different in PCG algorithm?
Other things that might affect results...
\fi



==> old_proof.tex <==

\begin{theorem}
In exact arithmetic, PCG for the solution of \cref{eq:Ax=b} with $P$ as a 
preconditioner converges in at most one more iteration than when using
$\Palpha$.
\end{theorem}
\begin{proof}
For any $c>0$, CG will converge for the system $cIx=f$ in one iteration in exact
arithmetic. We therefore set up a system where we scale both sides by $\alpha$.
For brevity, let $\tilde b = \Palpha\invhalf b$ and
\[
\tilde A = \alpha^\half \Palpha\invhalf A\Palpha\invhalf \alpha^\half.
\]
The preconditioned system is
\begin{subequations}
\begin{align}
& \tilde A z = \tilde b,\label{eq:preconditioned_system:Palpha}\\
& \Palpha^\half x = z.
\end{align}
\end{subequations}
We let $\tilde A = \mathsf{U}\Pi\mathsf{U}\transp$ denote an eigendecomposition,
and recall $\tilde E = VDV\Hermitian + W\Theta W\Hermitian$. The eigenvalues
$\Pi$ are given by
\begin{align*}
\pi_i
& = \lambda_i(\alpha(\alpha WW\Hermitian + V(I_r + D)V\Hermitian)\inv(I + \tilde E))\\
& = \begin{cases}
\alpha \qquad \text{if} & i \in \BregmanIndexSet{X},\\
1 + \theta_i & \text{otherwise}.
\end{cases}
%, \quad i=1,\ldots,n.
\end{align*}
We have the eigenvalue $1$ with a multiplicity of at least $r$.

The $k^\textnormal{th}$ iterate, $z_k$ of CG applied to
\cref{eq:preconditioned_system:Palpha} satisfies
\[
\| z_k - z \|_{M}^2 = \inf_{\substack{q\in\Polyk\\ q(0) = 1}} \Big\{ \frac{q(\alpha)^2}{\alpha}\sum_{i\in\BregmanIndexSet{X}} (\mathsf{u}_i\Hermitian \tilde b)^2 + \sum_{i\not\in\BregmanIndexSet{X}}^n \frac{q(1 + \pi_i)^2}{1 + \pi_i} (\mathsf{u}_i\Hermitian \tilde b)^2 \Big\}.
\]
How we consider a specific choice of $\alpha$, namely when $\alpha$ coincides with
one of the eigenvalues $1 + \pi_i$, $i\not\in\BregmanIndexSet{X}$. Let $\hat \alpha$
denote one such choice. Then,
\begin{align*}
\| z_k - z \|_{\tilde A}^2 %= & \inf_{\substack{q\in\Polyk\\ q(0) = 1}} \Big\{ \frac{q(\alpha)^2}{\alpha}\sum_{i\in\BregmanIndexSet{X}} (\mathsf{u}_i\Hermitian \tilde b)^2 + \sum_{i\not\in\BregmanIndexSet{X}}^n \frac{q(1 + \pi_i)^2}{1 + \pi_i} (\mathsf{u}_i\Hermitian \tilde b)^2 \Big\}\\
\geq & \inf_{\substack{q\in\Polyk\\ q(0) = 1}} \Big\{ \frac{q(\hat \alpha)^2}{\hat \alpha}\sum_{i\in\BregmanIndexSet{X}} (\mathsf{u}_i\Hermitian \tilde b)^2 + \sum_{i\not\in\BregmanIndexSet{X}}^n \frac{q(1 + \pi_i)^2}{1 + \pi_i} (\mathsf{u}_i\Hermitian \tilde b)^2 \Big\}\\
\geq & \inf_{\substack{q\in\Polynomials{k+1}\\ q(0) = 1}} \Big\{ \frac{q(\hat \alpha)^2}{\hat \alpha}\sum_{i\in\BregmanIndexSet{X}} (\mathsf{u}_i\Hermitian \tilde b)^2 + \sum_{i\not\in\BregmanIndexSet{X}}^n \frac{q(1 + \pi_i)^2}{1 + \pi_i} (\mathsf{u}_i\Hermitian \tilde b)^2 \Big\}\\
= & \| z_{k+1} - z \|_{\tilde A}^2.
\end{align*}
In other words, $\alpha$ represents another degree of freedom, and if this is chosen to 
\end{proof}

Let $\alpha$ be such that it lies in the interval given in \cref{eq:alpha:interval}
but does not coincide with any of the eigenvalues $\lambda_i(P\inv A)$, $i=1,\ldots,n$.
Suppose that PCG with $P_\alpha$ converges in $k>1$ iterations for the
system $Ax=b$, and let $\lambda = \lambda_i(P\inv A)$ denote any eigenvalue $i=1,\ldots,n$.\\
Then, PCG will convergence using the preconditioner $P_\lambda$ in no fewer than $k-1$ iterations for any  $i=1,\ldots,n$.

Choosing $\alpha$ to coincide with one remaining root can at most reduce the number of
iterations by one. %.. At most can choose $\alpha$ as one of the remanining eigenvalues, reduces the number of iterations by 1. 
We know the iteration error at iterate $k$ satisfies
\[
e^k = x^k - x^0 = P_k(HA) e^0,
\]
where $P_k$ is a polynomial of order $k$ with $P_k(0)=1$.
This means that PCG terminates after $q(HA, e^0)$ steps, where this quantity is
 given by the minimal polynomial to $HA$ and $e^0$, i.e., the smallest polynomial
 which annihilates $HA$.\\




\textbf{OLD STUFF}
\begin{subequations}\label{eq:zall}
\begin{align}
\| z_k - z \|_{M}^2
& = \inf_{\substack{q\in\Polyk\\ q(0) = 1}} \Big\{ \frac{q(1)^2}{1}\sum_{i\in\BregmanIndexSet{\tilde E}} (\mathsf{u}_i\Hermitian \tilde b)^2 + \sum_{i\not\in\BregmanIndexSet{\tilde E}} \frac{q(\frac{1 + \pi_i}\alpha)^2}{\frac{1 + \pi_i}\alpha} (\mathsf{u}_i\Hermitian \tilde b)^2 \Big\}\label{eq:zinf}\\
& = \frac{q^\star_\alpha(1)^2}{1}\sum_{i\in\BregmanIndexSet{\tilde E}} (\mathsf{u}_i\Hermitian \tilde b)^2 + \sum_{i\not\in\BregmanIndexSet{\tilde E}} \frac{q^\star_\alpha(\frac{1 + \pi_i}\alpha)^2}{\frac{1 + \pi_i}\alpha} (\mathsf{u}_i\Hermitian \tilde b)^2\label{eq:zinf:opt}\\
& =: J(q^\star_\alpha, \alpha).
\end{align}
\end{subequations}
where $q^\star_\alpha$ is the minimising polynomial.
We introduce $J$ since we want to reason about the minimising polynomial 
$q^\star_\alpha$ (which depends on $\alpha$) and the value of the objective
function if we were to change $\alpha$ to, say, $\hat \alpha$ (but not 
$q^\star_\alpha$!) which is given as argument to the polynomial in the 
second term of \cref{eq:zinf:opt}.\\

Since $\alpha$ is considered fixed when optimising over the polynomials
above, we cannot say that 
\[
J(q^\star_\alpha, \alpha) \geq J(q^\star_\alpha, \hat \alpha)
\]
for some other value $\hat\alpha$. If $q^\star_\alpha$ has a
root in $\frac{1 + \pi_i}\alpha$, there is no reason it should have a root
in $\frac{1 + \pi_i}{\hat\alpha}$. While it is true that we can choose
$\hat\alpha$ in such a way that $q^\star_\alpha(\frac{1 + \pi_i}{\hat \alpha})
= 0$ for some $i$, the choice of $\hat \alpha$ affects \emph{all} the $n-r$ 
eigenvalues in \cref{eq:zinf:opt}. As a result, we could make the
contributions $q^\star_\alpha(\frac{1 + \pi_j}{\hat \alpha})$ much larger for the 
remaining $j\neq i$.\\

As a first step, we need to manipulate \cref{eq:zinf} so we can remove $\alpha$
from the "inside" of $q$. We can use
\[
\mathcal{K}_k(M,\tilde b) = \mathcal{K}_k(\alpha M,\tilde b).
\]
\textcolor{red}{NEW APPROACH FROM THIS POINT}\\

Let us write
\[
I + \tilde E = I + VDV\Hermitian + W\Theta W\Hermitian.
\]
We can verify (using $WW\Hermitian = I - VV\Hermitian)$ that
\[
P\inv A = I + Q\invHermitian W \Theta W\Hermitian Q\Hermitian.
\]
\[
\alpha \Palpha\inv A = I + Q\invHermitian W \Theta W\Hermitian Q\Hermitian + (1-\alpha)Q\invHermitian VV\Hermitian Q\Hermitian.
\]
From which we get
\[
\mathcal{K}_k(P\inv A,\tilde b) = \mathcal{K}_k(I + Q\invHermitian W \Theta W\Hermitian Q\Hermitian ,\tilde b) = \mathcal{K}_k(Q\invHermitian W \Theta W\Hermitian Q\Hermitian ,\tilde b), 
\]
and
\begin{align*}
\mathcal{K}_k(\Palpha\inv  A,\tilde b)
& = \mathcal{K}_k(\alpha\Palpha\inv  A,\tilde b)\\
& = \mathcal{K}_k(I + Q\invHermitian W \Theta W\Hermitian Q\Hermitian + (1-\alpha)Q\invHermitian VV\Hermitian Q\Hermitian,\tilde b)\\
& = \mathcal{K}_k(Q\invHermitian W \Theta W\Hermitian Q\Hermitian + (1-\alpha)Q\invHermitian VV\Hermitian Q\Hermitian,\tilde b).
\end{align*}
We have 
\begin{align*}
\big(Q\invHermitian W \Theta W\Hermitian Q\Hermitian\big) \big((1-\alpha)Q\invHermitian VV\Hermitian Q\Hermitian\big)
& = 
(1-\alpha) \big(Q\invHermitian W \Theta W\Hermitian Q\Hermitian\big) \big(Q\invHermitian VV\Hermitian Q\Hermitian\big)\\
& = 
(1-\alpha) Q\invHermitian W \Theta W\Hermitian Q\Hermitian Q\invHermitian VV\Hermitian Q\Hermitian\\
& = 
(1-\alpha) Q\invHermitian W \Theta W\Hermitian VV\Hermitian Q\Hermitian\\
& = 0
\end{align*}
since
\[
W\Hermitian V = 0.
\]
As a result, the Krylov space $\mathcal{K}_k(\Palpha\inv  A,\tilde b)$ is
\begin{align*}
\mathcal{K}_k(\Palpha\inv  A,\tilde b)
& = \text{span}\Big\{\tilde b,
%\Big(Q\invHermitian W \Theta W\Hermitian Q\Hermitian \Big)\tilde b + \Big((1-\alpha)Q\invHermitian VV\Hermitian Q\Hermitian \Big)\tilde b, \\
\ldots ,\Big(Q\invHermitian W \Theta W\Hermitian Q\Hermitian \Big)^{k-1}\tilde b + \Big((1-\alpha)^{k-1}Q\invHermitian VV\Hermitian Q\Hermitian \Big)\tilde b\Big\}.
\end{align*}
The Krylov space $\mathcal{K}_k(P\inv  A,\tilde b)$ is
\begin{align*}
\mathcal{K}_k(P\inv  A,\tilde b)
& = \text{span}\Big\{\tilde b, \ldots ,\Big(Q\invHermitian W \Theta W\Hermitian Q\Hermitian \Big)^{k-1}\tilde b\Big\}.
\end{align*}
It would appear
\[
\mathcal{K}_k(P\inv  A,\tilde b) \subseteq \mathcal{K}_k(\Palpha\inv  A,\tilde b),
\]
with equality when $\alpha=1$. If we set $\alpha = 1 - \beta$, for some $\beta$, then
\[
\mathcal{K}_k(\Palpha\inv  A,\tilde b) = \mathcal{K}_k(\beta\inv Q\invHermitian W \Theta W\Hermitian Q\Hermitian +Q\invHermitian VV\Hermitian Q\Hermitian,\tilde b).
\]
We can chose $\beta$ as one of the diagonals of $\Theta$, i.e. one of the "remaining"
eigenvalues of the preconditioned matrix, but I am not sure how to use this observation.

\begin{align}
\| z_k - z \|_{M}^2
& = \inf_{w\in\mathcal{K}_k(\alpha M,\tilde b)}  \| w - z \|_{M}^2\\
& = \inf_{\substack{p\in\Polynomials{k-1}}} \Big\{ \half \|p(\alpha\Pi)\tilde b - \Pi\inv\tilde b\|_M^2\Big\}\\
& = \inf_{\substack{p\in\Polynomials{k-1}}} \half \sum_{i=1}^n (\mathsf{u}_i\Hermitian \tilde b)^2 \frac{(1 - \pi_ip(\alpha \pi_i))^2}{\pi_i}\\
& = \inf_{\substack{p\in\Polynomials{k-1}}} \half 
\sum_{i\in\BregmanIndexSet{\tilde E}} 
(\mathsf{u}_i\Hermitian \tilde b)^2 (1-p(\alpha))^2  + \sum_{i\not\in\BregmanIndexSet{\tilde E}} 
(\mathsf{u}_i\Hermitian \tilde b)^2 
\frac{(\alpha - (1+\theta_i)p(1+\theta_i))^2}{\alpha}
\end{align}
TBC (unless we find an error)...

\vspace{4cm}
Fast-forwarding a bit, I think we can formulate 
\cref{eq:zall} as 
\begin{align}
\| z_k - z \|_{M}^2
& = \inf_{\substack{p\in\Polynomials{k-1}}} \Big\{ \frac{(1 - p(\alpha)^2}{1}\sum_{i\in\BregmanIndexSet{\tilde E}} (\mathsf{u}_i\Hermitian \tilde b)^2 + \sum_{i\not\in\BregmanIndexSet{\tilde E}} \frac{\alpha\inv (\alpha - (1+\theta_i)p(1+\theta_i))^2}{\frac{1 + \pi_i}\alpha} (\mathsf{u}_i\Hermitian \tilde b)^2 \Big\}\label{eq:zinf}\\
& = \frac{q^\star_\alpha(1)^2}{1}\sum_{i\in\BregmanIndexSet{\tilde E}} (\mathsf{u}_i\Hermitian \tilde b)^2 + \sum_{i\not\in\BregmanIndexSet{\tilde E}} \frac{q^\star_\alpha(\frac{1 + \pi_i}\alpha)^2}{\frac{1 + \pi_i}\alpha} (\mathsf{u}_i\Hermitian \tilde b)^2\label{eq:zinf:opt}\\
& =: J(q^\star_\alpha, \alpha).
\end{align}


\vspace{3cm}
How we consider a specific choice of $\alpha$, namely when $\alpha$ coincides with
one of the eigenvalues $1 + \pi_i$, $i\not\in\BregmanIndexSet{\tilde E}$. Let $\hat \alpha$
denote one such choice. Then,
\begin{align*}
\| z_k - z \|_{M}^2 %= & \inf_{\substack{q\in\Polyk\\ q(0) = 1}} \Big\{ \frac{q(\alpha)^2}{\alpha}\sum_{i\in\BregmanIndexSet{\tilde E}} (\mathsf{u}_i\Hermitian \tilde b)^2 + \sum_{i\not\in\BregmanIndexSet{\tilde E}} \frac{q(1 + \pi_i)^2}{1 + \pi_i} (\mathsf{u}_i\Hermitian \tilde b)^2 \Big\}\\
\geq & \inf_{\substack{q\in\Polyk\\ q(0) = 1}} \Big\{ \frac{q(\hat \alpha)^2}{\hat \alpha}\sum_{i\in\BregmanIndexSet{\tilde E}} (\mathsf{u}_i\Hermitian \tilde b)^2 + \sum_{i\not\in\BregmanIndexSet{\tilde E}} \frac{q(1 + \pi_i)^2}{1 + \pi_i} (\mathsf{u}_i\Hermitian \tilde b)^2 \Big\}\\
\geq & \inf_{\substack{q\in\Polynomials{k+1}\\ q(0) = 1}} \Big\{ \frac{q(\hat \alpha)^2}{\hat \alpha}\sum_{i\in\BregmanIndexSet{\tilde E}} (\mathsf{u}_i\Hermitian \tilde b)^2 + \sum_{i\not\in\BregmanIndexSet{\tilde E}} \frac{q(1 + \pi_i)^2}{1 + \pi_i} (\mathsf{u}_i\Hermitian \tilde b)^2 \Big\}\\
= & \| z_{k+1} - z \|_{M}^2.
\end{align*}



==> rla.tex <==
\section{Approximations using randomised linear algebra}\label{sec:rla}

%\newpage
%Let $\widehat B(M) = \frac{\frac1n \tracexnys{M}}{\widehat{\det}(M)^{1/n}}$ denote an
%approximation of Kaporin's condition 
%Let $\widehat B(M) = \frac{\frac1n \tracexnys{M}}{\widehat{\det}(M)^{1/n}}$ denote an
%\newpage

Given the bounds in \cref{sec:convergence_results,sec:superlinear}, good
approximations of $\BCond{M}$, $\KCond{M}$ and $\BregmanLogDet(A,\Palpha)$ 
may be of use in practice. However, these terms involve the trace and
determinant of the preconditioned matrix, which can be computationally 
burdensome or impractical to compute numerically.\\

% Trace estimation
Trace estimation is a set of methods for approximating the trace of a matrix $M$.
% Hutch++, etc. here.
Since $\ln\det M = \trace{\ln M}$, we can use trace estimation to approximate all of
the constituent terms of $\BCond{M}$, $\KCond{M}$ and $\BregmanLogDet(A,P)$.
In this section, we discuss \emph{randomised} approach to trace estimation with applications
to estimating these quantities. Several alternatives exist, see \cite{persson2022improved}
and the references therein. Randomised linear algebra (RLA) is a family of techniques in 
linear algebra that leverages randomness to approximate large-scale problems that may 
otherwise be computationally infeasible \cite{halko2011finding,martinsson2020randomized}.
Such methods are useful for handling large datasets or matrices, where traditional methods
become too slow or memory-intensive.

%Since randomness is involved, the results are approximate,
%but error can often be controlled.

% Computational cost of methods
%The computational cost of XNysTrace is $O(x)$, and stochastic Lanczos method is $O(x)$.

\subsection{Approximation of Kaporin's condition number}

By \cref{eq:lnK_expanded}, a randomised approximation of $\KCond{M}$ for some 
preconditioned matrix $M\in\Snpp$ amounts to approximating $\trace{M}$ and $\trace{\ln(M)}$.
We use the following notation to denote an approximation of $\trace{\ln(M)}$ using
stochastic Lanczos quadrature (SLQ) \cite{ubaru2017fast}:
%\footnote{Matlab code for this method is available \url{https://github.com/Shashankaubaru/SLQ}.} 
\[
\slogdet{M} \approx \trace{\ln(M)}. %\ln\det M.
\]
SLQ employs the Lanczos procedure\footnote{Golub-Kahan bidiagonalisation can also be used,
see the discussion in \cite{ubaru2017fast}.} to produce an orthonormal basis $U_m$ for the Krylov
subspace
\[
\linearspan{v_0,\ldots,M^{m-1} v_0}
\]
and a tridiagonal matrix $T_m$ 
(where $v_0$ is a random starting vector with $\|v_0\|_2 = 1$) such that
\[
U_m\Hermitian M U_m = T_m.
\]
The subspace dimension $m$ is chosen such that the eigenvaluedecomposition 
\[
T_m = \mathsf{V}_m \Pi_m \mathsf{V}_m\Hermitian \in \mathbb{R}^{m\times m}
\]
is not prohibitive to compute. $\slogdet{M}$ can then be computed by using by 
averaging $\trace{\ln \Pi_m}$ for $n_v$ different random starting vectors $v_0$:
\[
\tracexnys{\ln M} := \frac{n}{n_v} \sum_{i=1}^{n_v} ...
\]
see \cite[Equation 9]{ubaru2017fast}.
An approximation $\tracexnys{M} = \trace{\Pi_m}$ of the trace $\trace{M}$ can be obtained simultaneously 
for the same amount of computing effort. For $m$ steps Lanczos method for $n_v$ different
starting vectors, the computational cost of SLQ is $O\big((\mathsf{nnz}(M)m + nm^2)n_v\big)$,
where $\mathsf{nnz}(M)$ is the number of nonzeros of $M$. 
\Cref{eq:hatalpha} could also be approximated using the so-called XNysTrace method 
\cite{epperly2024xtrace} for stochastic trace estimation of Hermitian positive semidefinite 
matrices.\\

By combining the methods above, we arrive at an approximation $\KCondApprox{M}\approx\KCond{M}$:
\begin{equation}\label{eq:KCondApprox}
\KCondApprox{M} = \frac{\frac{1}{n}\trace{\Pi_m}}{\tracexnys{\ln M}}
\end{equation}
which, when $M$ is a preconditioned matrix, can be used as a surrogate for $\KCond{M}$
in the PCG convergence bounds presented in \cref{sec:superlinear}. We now explore these
approximations numerically, and pursue a theoretical treatment in a sequel.\\

We select matrices from SuiteSparse \cm. These are shown in \cref{table:test_matrices},
and are of relatively small size. The aim here is to study the behaviour of the 
approximation $\KCondApprox{M}$ in \cref{eq:KCondApprox} and compare it with the exact quantity 
$\KCond{M}$.

\input{test_matrices.tex}

\subsection{Stochastic estimation of $\alpha$ and associated quantities}

While \cref{thm:iteration_alpha} shows that the choice of $\alpha$ does not
affect the PCG algorithm, it may be useful to obtain an approximation $\hat\alpha \approx 
\alpha^\star$ in order to compute $\ln \KCond{P_{\hat\alpha}\inv A}$.
By \cref{eq:alpha}, a good estimate of $\trace{P\inv A}$ is required (recall that $P$, given
in \cref{eq:Bregman_preconditioner}, is a precursor to $\Palpha$) in order to compute an
approximation $\hat\alpha$ of $\alpha^\star$. By an argument
similar to the one presented in the previous section and \cref{eq:BregmanEqualslogKaporin},
an approximation of $\BregmanLogDet(A, \Palpha)$ also requires approximations of
$\trace{\ln(P\inv A)}$. Given $P$ in \cref{eq:Bregman_preconditioner}, we can therefore
an approximation $\Phatalpha \approx \Palphastar$ given by
\[
\Phatalpha = Q(\hat\alpha(I - VV\Hermitian) + V(I_r + D)V\Hermitian)Q\Hermitian,
\]
where
\begin{equation}\label{eq:hatalpha}
\hat\alpha = \frac{\tracexnys{P\inv A}-r}{n-r}
\end{equation}
and $\tracexnys{P\inv A}$ has been computed along with $\slogdet{P\inv A}$ using the
SLQ method described above. Recall that the latter is necessary to compute
an approximation $\widehat{\BregmanLogDet}(A,\Phatalpha)$ of $\BregmanLogDet(A,\Phatalpha)$:
\[
\BregmanLogDet(A,\Phatalpha) \approx \widehat{\BregmanLogDet}(A,\Phatalpha) := - \tracexnys{\ln(P\inv A)} + (n-r)\ln(\hat\alpha),
\]
which can be used as a surrogate for $\BregmanLogDet(A,\Palpha)$ in the PCG convergence
bounds presented in \cref{sec:superlinear}.\\

\Cref{eq:hatalpha} could also be approximated using the so-called 
XNysTrace
%\footnote{XNysTrace Matlab code is available at \url{https://github.com/eepperly/XTrace}.} 
\cite{epperly2024xtrace} method for
stochastic trace estimation of Hermitian positive semidefinite matrices. While SLQ is
also necessary to compute $\BregmanLogDet(A,\Phatalpha)$, the matrix-vector 
products required for XNysTrace may be stored and reused in the SLQ algorithm.

%\iffalse
\subsection{Randomly Pivoted Cholesky \& Nyström Preconditioner}

Let $\tracexnys{M}$ denote the output from the Hutch++ procedure.
From \cite[Theorem 1]{hutchpp} we have
\[
(1 - \epsilon)\trace{M} \leq \tracexnys{M} \leq (1 + \epsilon)\trace{M},
\]
where $\epsilon$ depends on the chosen rank.\\

Let $\Gamma \approx \ln\det{M}$ be the output of SLQ, and set
\[
\KCondApprox{M} = \frac{\big(\frac{1}{n} \tracexnys{M}\big)^n}{e^\Gamma} \approx \KCond{M}.
\]

\begin{proposition}
    
\end{proposition}
\begin{proof}
By \cite[Theorem 4.1]{ubaru2017fast}, we have, with some probability,
\begin{equation}\label{eq:bound4}
|\ln\det{M} - \Gamma| \leq  \epsilon |\ln\det{M}|.
\end{equation}

Therefore,
\begin{align}
\Gamma
& \leq |\Gamma - \ln\det{M}| + |\ln\det{M}|\nonumber\\
& \leq \epsilon |\ln\det{M}| + |\ln\det{M}|\nonumber\\
& = (1 + \epsilon)|\ln\det{M}|.\label{eq:bound1}
\end{align}
To show
\cref{eq:bound3} holds, we need
\[
\Gamma \leq \ln\det{M}.
\]
\Cref{eq:bound1} establishes a link between $\Gamma$ and $\ln\det{M}$. However,
\begin{equation}\label{eq:bound2}
\ln \det M \leq |\ln\det M|.
\end{equation}
In other words, it does not appear easy/possible  to use \cref{eq:bound1} and \cref{eq:bound2} to establish the desired inequality
\[
\Gamma \leq \ln\det{M}.
\]
So \cref{eq:bound4} does not appear to help us due to the absolute values present.
\end{proof}

The aim is to prove
\begin{equation}\label{eq:bound3}
\KCond{M} \leq \KCondApprox{M}.
\end{equation}
%\fi


==> rubbish.tex <==
\appendix

\section{Miscellaneous}

\textbf{On the sublinear and superlinear rate of convergence of conjugate gradient methods (Axelsson, Kaporin '00)}

 
The authors discuss the three phases of PCG:
\begin{enumerate}
\item First phase PCG acts mainly on the information of the initial iteration error (a rapid initial convergence but of short duration is normally seen).
\item Middle phase: the method is influenced mainly by the spectral condition number and eventually, when a sufficient number of extreme eigenvalue components have been essentially damped out.
\item Final phase: the method enters the superlinear convergence phase.
\end{enumerate}

They define
\[
\kappa(A, x) = \frac{\|Ax\|}{\|x\|} \|A^{-1}\|,
\]
and 
\[
\kappa(A) = \|A\| \|A^{-1}\|.
\]
Then,
\[
\kappa(A, x) \leq \frac{\sup_x \frac{\|Ax\|}{\|x\|}}{\inf_x \frac{\|Ax\|}{\|x\|}} = \kappa(A).
\]
They also define some weird condition numbers $G(A,x)$ and $F(A,x)$.\\

\subsection{Fixed Sparsity Pattern Approaches}

We study preconditioning of the nonsingular system
\[
Ax = b.
\]
Preconditioning is often a requirement for acceleration of iterative
methods. We therefore seek a preconditioning matrix $G$ and solve
\[
GAx = Gb.
\]

The main idea is to fix a sparsity pattern $\SparsityPattern$ for $G$:
\[
G_{ij} = 0, \quad (i,j) \not\in\SparsityPattern.
\]

Fast sparse approximate inverse preconditioners were studied in \cite{kolotilina1993factorized}, where a..\\

\textbf{Explicit formula given sparsity pattern?}

\subsection{Simple preconditioner}
\[
S = B\transp A\inv B.
\]
We set
\[
S_\textbf{SIMPLE} = QQ\transp = B\transp \diag(A)\inv B = B\transp \diag(A)^{-1/2}\diag(A)^{-1/2} B,
\]
i.e. $Q = B\transp \diag(A)^{-1/2}$.
With a low-rank term:
\[
S_\textbf{SIMPLE}^r = Q(I + G_r)Q\transp,
\]
where $G_r$ is a low-rank truncation of
\begin{align*}
G = Q\inv(S - S_\textbf{SIMPLE})Q\invtransp
& = Q\inv B\transp (A\inv - \diag(A)\inv) B Q\invtransp\\
& = (B\transp \diag(A)^{-1/2})\inv B\transp (A\inv - \diag(A)\inv) B (B\transp \diag(A)^{-1/2})\invtransp\\
& = (B\transp \diag(A)^{-1/2})\inv B\transp A\inv B (B\transp \diag(A)^{-1/2})\invtransp - I.
\end{align*}
If $B$ is square,
\begin{align*}
G = Q\inv(S - S_\textbf{SIMPLE})Q\invtransp
& = \diag(A)^{1/2} A\inv (\diag(A)^{1/2})\transp - I,
\end{align*}
so this matrix is \emph{hollow}. Therefore, the trace of
$G$ is zero, and
\[
\lambda_i(G) \in [0, \sum_{j=1}^n |G_{ij}|)
\]
although this is likely not useful in practice. 


~\\[2cm]
\todo{Bregman projections?}
\subsection{Operator Trigonometry}

In \cite{kaporin1990alternative} there is mention of angles 
between matrices.

We also note that $K(M)\geq 1$, and $K(M)=1$ only when
all the eigenvalues are equal.
\[
\theta = \cos(K(M))\inv.
\]

\begin{example}[Diagonal matrices]
We provide a simple example where both $A$ and $P$ are diagonal matrices.
Suppose $A = \sum_{i=1}^n \alpha_i e_ie_i\transp$ and for some set
$J\subset \{1,\ldots,n\}$ with $\# J = r$,
\[
P = \sum_{i\not\in J}  \beta e_ie_i\transp + \sum_{i\in J} (\gamma_i - \beta)e_ie_i\transp.
\]
The second term is a low-rank matrix, with $\# J$ degrees of freedom expressed
through $\gamma_i$. The remaining eigenvalues of the $P$ are determined by $\beta$.
Minimising $\BregmanLogDet(A, P)$ as a function of $\beta$, $J$ and $\gamma$ is
a combinatorial problem. From the expression
\begin{align*}
\BregmanLogDet(A, P)
& = \trace{P\inv A} - \log\det{P\inv A} - n\\
& = \sum_{i\not\in J} \frac{\alpha_i}{\beta} + \sum_{i\in J} \frac{\alpha_i}{\gamma_i} - \log\det(A) + (n-r)\log\beta + \sum_{i\in J} \log\gamma_i - n
\end{align*}
it is easy to see that any minimiser must satisfy
\begin{subequations}
\begin{align}
\gamma_i = \alpha_i,\quad i\in J,\label{eq:diagonal_matrices:gamma}\\
\beta = \sum_{i\not\in J} \frac{\alpha_i}{n-r}\label{eq:diagonal_matrices:beta}.
\end{align}
\end{subequations}
As a result, if a subset of the eigenvalues of the preconditioned matrix $M$
are set to unity (by the choice in \cref{eq:diagonal_matrices:gamma}), then 
the remaining eigenvalues fo $M$ must be scaled by the arithmetic mean of the
remaining eigenvalues of for $M$ to minimise Kaporin's condition number.
\end{example}




\input{background}
\input{trigonometry}
\section{Alternating projections}

Diagonal + Low rank preconditioner, alternating projections?

\subsection{Constraint manifold}

\newcommand{\Symrn}{S(r,n)}
In this section we investigate the following manifold \cite{helmke1995critical}:
\begin{equation}\label{eq:manifold:Symrn}
\Symrn = \{ X \in \Rnn\given X = X\transp, \rank{X} = r \},
\end{equation}
with tangent space at $X\in\Symrn$:
\begin{equation}\label{eq:tangent_space:Symrn}
T_X \Symrn = \{\Delta X  + X\Delta\transp\given \Delta\in\Rnn\}.
\end{equation}

\todo{Is the set $\{X\in\Sn,\; \rank X = r. \}$ a submanifold of $M$?}\\
\todo{Is the set $\{I + X\in\Sn,\; \rank X = r. \}$ a submanifold of $M$?}\\

We define
\[
C_r = \{ (I + X)\inv\in\Sn,\; \rank X \leq r. \},
\]
\begin{theorem}
$C_r$ is a flat submanifold of $M$.
\end{theorem}
\begin{proof}
First we show that $C_r$ is a submanifold of $M$. This is trivial 
\end{proof}
Note that we can write any rank $r$ matrix $X\in\Sn$ as
\[
X = F D F\transp, \quad F\in\Rnr, D \in\Rrr.
\]
Thanks to the Sherman-Morrison-Woodbury identity we have
\[
(I + X)\inv = I - F(D\inv + F\transp F)\inv F\transp,
\]
so $C_r$ is isomorphic to $C_r\inv = \{ W\inv \given W \in C_r\}$.\\

We now consider the following problem, where $A = I + G\in\Snpp$.
\begin{align}
\min_{P\in\Snpp} \quad & \BregmanLogDet(A, P)\\
\subto\quad
& P = I + X\\
& \rank{X} \leq r.
\end{align}

\subsection{Gradient}

Recall the following definition:

\begin{definition}[Riemannian gradient]\label{def:Riemannian_gradient}
Let $J : \mathcal{M} \rightarrow \mathbb{R}$ denote a function on a manifold $\mathcal{M}$.
The Riemannian gradient, $\nabla_X J \in T_X \mathcal{M}$ denotes the gradient of $J$ at
$X$ given some direction $V \in T_X \mathcal{M}$. Let $\phi_{X, V}(t)$ denote a geodesic
emanating from $X$ in the direction of $V$. Then $\nabla_X J$ is the unique tangent vector
satisfying
\[
\langle V, \nabla_X J\rangle_X = \frac{\partial}{\partial t} J(\phi_{X, V}(t))|_{t=0}.
\]
\end{definition}

The Riemannian gradient is, thanks to \cref{def:Riemannian_gradient},
\[
\nabla_X f(X) = ...% (I + X) \log{(I + G)\inv (I + X)} = - (I + X) \log{(I + X)\inv (I + G)}.
\]
For each $X\in\Symrn$, the projection $\Pi_{T_X \Symrn} : ? \rightarrow \Symrn$ onto the tangent space $T_X \Symrn$ is defined as:
\[
\Pi_{T_X \Symrn} \Big[ M \Big] = something
\]

\subsection{Algorithm}

We therefore come to the following optimisation algorithm:
\begin{enumerate}
    \item Select candidate $X_0$
    \item $k \gets 0$
    \item Compute the gradient $h_k = \Pi_{T_X \Symrn} \Big[\nabla_X f(X_k)\Big]$
    \item Apply exponential map $X_{k+1} = \text{Exp}_{X_k}(- \alpha h_k)$, for some $\alpha >0$
    \item $k \gets k + 1$
    \item If not converged, go to step 3
\end{enumerate}
\subsection{General diagonal scaling}

Let $\DiagSnpp$ denote the diagonal matrices of $\Snpp$.

\begin{subequations}\label{eq:Bregman_preconditioner:scaling:general}
\begin{align}
\min_{\substack{D\in\DiagSnpp,\\K\in\Sn}} \quad & \BregmanLogDet(D(I + G)D, I + K)\\
\subto\quad
& I + K \in \Snpp,\\
& K = U\\
& \rank K \leq r.
\end{align}
\end{subequations}

Let \[
\BregmanLogDet(D(I + G)D, I + K) = \trace{(I+K)\inv D(I+G)D} - \ln\det\big((I+K)\inv D(I+G)D\big) - n = T_1 + T_2 - n.
\]
%We have
%\begin{align*}
%dT_1/dD = 2\trace{ADH dD},\\
%dT_2/dD = - 2\trace{D\inv dD},
%\end{align*}
%so any
A minimiser $D$ of \cref{eq:Bregman_preconditioner:scaling:general} must satisfy
\[
D_{ii}\inv = \big(ADH\big)_{ii}.
\]

\begin{remark}
We see that if $D = \beta I$, $\beta > 0$, then
\[
\beta^2 = \frac{n}{\trace{HA}},
\]
which is in agreement with the results of \cref{sec:constant:diagonal}.
\end{remark}

Define $F: \Realn \mapsto \Realn$ by
\[
F(D)_i = D_{ii}\inv - \big(ADH\big)_{ii}.
\]
It can be verified that
\[
F'(D)_i = - \big(D_{ii}^{-2} + A \odot H\big),
\]
where $\odot$ is the Hadamard (or Schur) product. Newton's method for
solving $F(D)=0$ can be written as
\begin{align*}
D^{k+1}
& = D^k - F'(D^k)\inv F(D^k)\\
& = D^k + \Big((D^k)^{-2} + A \odot H\Big)\inv \Big((D^k)^{-1} - \diag(A D^k H)\Big).
\end{align*}

A secant-type method such as Broyden's method can also be used. Such a 
scheme is, however, not feasible to implement in general for large matrices.

\todo{Limitation on sparsity pattern of $H$?}



\iffalse
We shall use 
XNysTrace for trace estimation and
use $\tracexnys{M}$ to denote an approximation of the trace of $M$:
\[
\tracexnys{M} \approx \trace{M}.
\]

\begin{theorem}[Bound on trace and log determinant using randomised methods]\label{thm:tracelogdet_estimates}
Let $M\in\Snpp$ and
\begin{align*}
& \tracexnys{M} \leq ...\\
& \log \det{M} \leq ...
\end{align*}
\end{theorem}
\begin{proof}
\end{proof}

\begin{corollary}[Bounds for $\BCond{M}$, $\KCond{M}$ and $\BregmanLogDet(A,P)$]
\begin{align*}
\BregmanLogDet(A,P) & \leq ...\\
\BCond{M} & \leq ...\\
\KCond{M} & \leq ...
\end{align*}

\end{corollary}
\begin{proof}
By \cref{thm:tracelogdet_estimates}, we obtain the estimate for the divergence.
Further ...
\begin{align*}
\ln \KCond{M} & = n\big( \ln(n\inv) + \ln\trace{M}\big) - \ln\det M.
\end{align*}
\end{proof}

%%%%%%%
$\alpha$ in \cref{eq:alpha} may 
\[
\alpha = \trace{P\inv A} = \mathbb{E}[\epsilon\transp P\inv A \epsilon] \approx \trace{\Omega P\inv A \Omega} =: \tilde\alpha.
\]

Influence of the trace normalisation: see notes.

\subsection{Numerical experiments with simulated data}

In this section, we provide a small numerical illustration of the effect of
the trace estimator above on the convergence estimates in \cref{something}
and PCG. We shall therefore simulate a preconditioned matrix $M$ with various 
dimension and spectral properties. We consider spectra for $M$ as depicted in
\cref{fig:rla:spectra}, with 

\begin{equation}\label{eq:spectrum}
\lambda_A(i) = \exp\{-(\alpha_A i/n  - c_A)^{\beta_A}\} + \kappa.
\end{equation}

\begin{table}[tbhp]
\footnotesize
    \caption{Parameters used to generate spectra of $M$. Visualisations of these spectra can be seen in Figure \ref{fig:rla:spectra}.}\label{table:rla:spectra}
    \centering
\begin{tabular}{|l|l|l|c|l|c|}\hline
$\alpha$ & $c$ & $\beta$ & $\kappa$ & \textbf{Description} & \textbf{Label}\\\hline
$0$ & $0$ & $0$ & $0.70$ & flat & 1 \\
$3.5$ & $0$ & $1.0$ & $0.05$ & exponential & 2\\
$4.0$ & $0.30$ & $4.5$ & $0.05$ & drop-off and fast decay & 3\\
$2.0$ & $0.25$ & $4.5$ & $0.05$ & drop-off at $n/2$ & 4\\\hline
\end{tabular}
\end{table}
\begin{figure}
    \centering
    \includegraphics[scale=0.4]{figures/spectra.pdf}
    \caption{Different choices of spectra for $A$ and $B$ using the parameters in Table \ref{table:AB_params}.}
    \label{fig:rla:spectra}
\end{figure}

\todoinline{Synthetic data: plot convergence of PCG along with the different asymptotic estimates.}

\todoinline{Same using randomised Nyström preconditioner (e.g. using their examples).}
\fi
